Rigorous mathematical optimization of synthetic hepatic vascular trees

In this paper, we introduce a new framework for generating synthetic vascular trees, based on rigorous model-based mathematical optimization. Our main contribution is the reformulation of finding the optimal global tree geometry into a nonlinear optimization problem (NLP). This rigorous mathematical formulation accommodates efficient solution algorithms such as the interior point method and allows us to easily change boundary conditions and constraints applied to the tree. Moreover, it creates trifurcations in addition to bifurcations. A second contribution is the addition of an optimization stage for the tree topology. Here, we combine constrained constructive optimization (CCO) with a heuristic approach to search among possible tree topologies. We combine the NLP formulation and the topology optimization into a single algorithmic approach. Finally, we attempt the validation of our new model-based optimization framework using a detailed corrosion cast of a human liver, which allows a quantitative comparison of the synthetic tree structure to the tree structure determined experimentally down to the fifth generation. The results show that our new framework is capable of generating asymmetric synthetic trees that match the available physiological corrosion cast data better than trees generated by the standard CCO approach.

==> input/math-fields.tex <==
% Math fields -- requires amsfonts

\newcommand{\field}{\mathbb}

% "natural" names
\newcommand{\complex}{\field{C}}
\newcommand{\quaternions}{\field{H}}
\newcommand{\naturals}{\field{N}}
\newcommand{\polynomials}{\field{P}}
\newcommand{\rationals}{\field{Q}}
\newcommand{\reals}{\field{R}}
\newcommand{\integers}{\field{Z}}

% alternative names
\newcommand{\numsetC}{\complex}
\newcommand{\numsetH}{\quaternions}
\newcommand{\numsetN}{\naturals}
\newcommand{\numsetQ}{\rationals}
\newcommand{\numsetR}{\reals}
\newcommand{\numsetZ}{\integers}

% short names
\makeatletter
\@ifundefined{C}{\newcommand{\C}{\complex}}
{\PackageInfo{math-fields}{Use \string\field{C} for complex numbers;
 \MessageBreak command \string\C\space already defined}{}}
\makeatother
\newcommand{\N}{\naturals}
\newcommand{\Q}{\rationals}
\newcommand{\R}{\reals}
\newcommand{\Z}{\integers}
\newcommand{\Poly}{\polynomials}% deprecated: NuMa scripts


==> input/math-graphs.tex <==
% Graph macros -- requires amsfonts and math-symbols

% Set of graph elements.
\newcommand{\graphset}{\mathbb}
\newcommand{\graphindex}{\tsb}% alternative: \tsp

\newcommand{\Graph}{\graphset{G}}
\newcommand{\Arcs}{\ensuremath{\graphset{A}}}
\newcommand{\Edges}{\graphset{E}}
\newcommand{\Nodes}{\graphset{V}}
\newcommand{\Vertices}{\Nodes}

\newcommand\Tree{\graphset{T}}
\newcommand\Level{\graphset{L}}
\newcommand\Leaves{\graphset{L}}

\newcommand{\node}{i}
\newcommand{\otherNode}{j}
\newcommand{\vertex}{v}
\newcommand{\otherVertex}{u}
\newcommand{\edge}{e}
\newcommand{\arc}{a}

\newcommand{\Arc}[1]{\Arcs\graphindex{#1}}
\newcommand{\Edge}[1]{\Edges\graphindex{#1}}
\newcommand{\Node}[1]{\Nodes\graphindex{#1}}
\newcommand{\Vertex}[1]{\Vertices\graphindex{#1}}

\newcommand{\BufNodes}{\Node{buf}}
\newcommand{\CtrlArcs}{\Arc{ctrl}}

\newcommand{\Junctions}{\Nodes_0}
\newcommand{\Sources}{\Nodes_+}
\newcommand{\Entries}{\Sources}
\newcommand{\Sinks}{\Nodes_-}
\newcommand{\Exits}{\Sinks}
\newcommand{\Heads}{\delta^+}
\newcommand{\Tails}{\delta^-}
\newcommand{\BoundaryNodes}{{\Nodes^\circ}}


\newcommand{\cardA}{\card{\Arcs}}
\newcommand{\cardE}{\card{\Edges}}
\newcommand{\cardN}{\card{\Nodes}}
\newcommand{\cardV}{\card{\Vertices}}

\newcommand{\IncMat}{E}% incidence matrix


==> input/math-std.tex <==
% Standard math definitions -- requires amsmath

\newcommand\const{\textup{const}}
\newcommand\qtext{\quad\text}
\newcommand\textq[1]{\text{#1}\quad}
\newcommand\qtextq{\quad\textq}
\newcommand\st{\textup{s.t.}}
\newcommand\stq{\st\quad}
\newcommand\qst{\quad\st}
\newcommand\qstq{\qst\quad}

\makeatletter
\newcommand\fcdot{\,\cdot\,}
\newcommand\ifgiven[3]{\def\fc@rg{#1}\ifx\fc@rg\empty#3\else#2\fi}
\newcommand\fcarg[1]{\ifgiven{#1}\fc@rg\fcdot}
\makeatother
\newcommand\abs[1]{\lvert\fcarg{#1}\rvert}
\newcommand\Abs[1]{\left\lvert#1\right\rvert}
\newcommand\tfracabs[2]{\abs{#1}/\abs{#2}}
\newcommand\fracabs[2]{\frac{\abs{#1}}{\abs{#2}}}
\newcommand\fracAbs[2]{\frac{\Abs{#1}}{\Abs{#2}}}
\newcommand\tabsfrac\tfracabs
\newcommand\absfrac\fracabs
\newcommand\Absfrac\fracAbs
\newcommand\card\abs
\newcommand\Card\Abs
\newcommand\ceil[1]{\lceil\fcarg{#1}\rceil}
\newcommand\Ceil[1]{\left\lceil#1\right\rceil}
\newcommand\defsep\colon% alternative: \mid
\newcommand\defset[3][\defsep]{\set{#2#1#3}}
\newcommand\Defset[3][\defsep]{\Set{#2#1#3}}
\newcommand\EEmult\cdot% alternative: \times
\newcommand\EE[1][\EEmult]{#1 10^}
\newcommand\floor[1]{\lfloor\fcarg{#1}\rfloor}
\newcommand\Floor[1]{\left\lfloor#1\right\rfloor}
\newcommand\Inv[1]{#1^{-1}}
\newcommand\HInv[1]{#1\ihr}% hermitian inverse
\newcommand\TInv[1]{#1\itp}% transpose inverse
\newcommand\norm[2][]{\lVert\fcarg{#2}\rVert\optsb{#1}}
\newcommand\Norm[2][]{\left\lVert#2\right\rVert\optsb{#1}}
\newcommand\tfracnorm[3][]{\norm[#1]{#2}/\norm[#1]{#3}}
\newcommand\fracnorm[3][]{\frac{\norm[#1]{#2}}{\norm[#1]{#3}}}
\newcommand\fracNorm[3][]{\frac{\Norm[#1]{#2}}{\Norm[#1]{#3}}}
\newcommand\tnormfrac\tfracnorm
\newcommand\normfrac\fracnorm
\newcommand\Normfrac\fracNorm
\newcommand\tfracnormpow[4][]{\norm[#1]{#2}^{#4}/\norm[#1]{#3}^{#4}}
\newcommand\fracnormpow[4][]{\frac{\norm[#1]{#2}^{#4}}{\norm[#1]{#3}^{#4}}}
\newcommand\fracNormpow[4][]{\frac{\Norm[#1]{#2}^{#4}}{\Norm[#1]{#3}^{#4}}}
\newcommand\pfrac[2]{\frac{\partial#1}{\partial#2}}
\newcommand\ppfrac[3]{\pfrac{^2#1}{#2\partial#3}}
\newcommand\set[1]{\{#1\}}
\newcommand\Set[1]{\left\{#1\right\}}
\newcommand\snorm[2][]{\lvert\!\lvert\!\lvert
  \fcarg{#2}\rvert\!\rvert\!\rvert\optsb{#1}}
\newcommand\Snorm[2][]{\left\lvert\!\left\lvert\!\left\lvert
  #2\right\rvert\!\right\rvert\!\right\rvert\optsb{#1}}
\newcommand\sprod[3][]{\langle\fcarg{#2},\fcarg{#3}\rangle\optsb{#1}}
\newcommand\Sprod[3][]{\left\langle#2,#3\right\rangle\optsb{#1}}

\newcommand\hrchar{H}
\newcommand\tpchar{T}
\newcommand\hr{^\hrchar}% hermitian transpose
\newcommand\tp{^\tpchar}
\newcommand\ihr{^{-\hrchar}}
\newcommand\itp{^{-\tpchar}}
\newcommand\tadj[1]{\mskip#1\thinmuskip}% adjust space
\newcommand\hra[1][0]{^{\tadj{#1}\hrchar}}
\newcommand\tpa[1][0]{^{\tadj{#1}\tpchar}}
\newcommand\ihra[1][0]{^{\tadj{#1}{-}\hrchar}}
\newcommand\itpa[1][0]{^{\tadj{#1}{-}\tpchar}}
\newcommand\tpfrac[2]{\tfrac{\partial#1}{\partial#2}}
\newcommand\tppfrac[3]{\tpfrac{^2#1}{#2\partial#3}}
\newcommand\without{\setminus\set}
\newcommand\Without{\setminus\Set}

\newcommand\lbound{-}
\newcommand\ubound{+}
\newcommand\splb{^{\lbound}}
\newcommand\spub{^{\ubound}}
\newcommand\sblb{_{\lbound}}
\newcommand\sbub{_{\ubound}}
\newcommand\bounds[1]{\ensuremath{[#1\splb,#1\spub]}}
\newcommand\Bounds[1]{\ensuremath{\left[#1\splb,#1\spub\right]}}

\newcommand\Strut{\rule[2.5555ex]{0pt}{0pt}}% ~1.1em
\newcommand\Hline{\hline\Strut}

\newcommand\optsb[1]{\ifgiven{#1}{_{#1}}{}}
\newcommand\optsp[1]{\ifgiven{#1}{^{#1}}{}}
\newcommand\optindex[1]{\ifgiven{#1}{,#1}{}}
\newcommand\optmathsb\optsb
\newcommand\optmathsp\optsp
\newcommand\opttextsb[1]{\optsb{\textup{#1}}}
\newcommand\opttextsp[1]{\optsp{\textup{#1}}}
\newcommand\optmathindex\optindex
\newcommand\opttextindex[1]{\optindex{\textup{#1}}}

\newcommand\define{\mathrel{{\mathop:}{=}}}
\newcommand\enifed{\mathrel{{=}{\mathop:}}}


==> input/math-symbols.tex <==
% Math symbols -- requires amsmath

% Redefine some macros in math mode. Keep text mode definitions.
\let\TeXbar\_   % underscore -> \bar
\let\TeXhat\^   % undefined  -> \hat
\let\TeXtilde\~ % undefined  -> \tilde
\let\TeXcolon\: % \tmspace+\medmuskip{.2222em} -> \colon
\makeatletter
\newcommand\mcs@cc[3]{\leavevmode\ifmmode#1{#3}\else#2{#3}\fi}
\renewcommand\_{\mcs@cc\bar\TeXbar}
\renewcommand\^{\mcs@cc\hat\TeXhat}
\renewcommand\~{\mcs@cc\tilde\TeXtilde}
\renewcommand\:{\mcs@cc\colon\TeXcolon\relax}
\makeatother
\PackageInfo{math-symbols}{Redefining
 \string\_, \string\^, \string\~, \string\: in math mode.
 \MessageBreak Keeping text mode definitions.
 \MessageBreak Saving original commands as \string\TeXbar, \string\TeXhat,
 \MessageBreak \string\TeXtilde, \string\TeXcolon}

\newcommand\0\emptyset
\newcommand\bigM{M}
\newcommand\bigO{O}
\newcommand\smallo{o}
\newcommand\oo\infty
\newcommand\ox\otimes
\newcommand\x\times

\newcommand\itxt{\textup}% text in math indices
\newcommand\tsb[1]{_{\itxt{#1}}}% text subindex
\newcommand\tsp[1]{^{\itxt{#1}}}% text superindex

\newcommand\boundary\partial
\newcommand\cond\kappa
\newcommand\condabs{\cond\tsb{abs}}\newcommand\abscond\condabs
\newcommand\condrel{\cond\tsb{rel}}\newcommand\relcond\condrel
\newcommand\convrad\rho
\newcommand\eps\epsilon
\newcommand\veps\varepsilon
\newcommand\epsM{\veps\tsb{M}}
\let\epsmach\epsM
\newcommand\specrad\rho
\newcommand\spectrum\sigma
\newcommand\uvec{\mathbf1}

% Some arrows.
\newcommand\larrow\leftarrow
\newcommand\rarrow\to% \rightarrow
\newcommand\swap\leftrightarrow
\newcommand\lrarrow\swap
\newcommand\Larrow\longleftarrow
\newcommand\Rarrow\longrightarrow
\newcommand\LRarrow\longleftrightarrow
\newcommand\xlarrow\xleftarrow
\newcommand\xrarrow\xrightarrow
\newcommand\lArrow\Leftarrow
\newcommand\rArrow\Rightarrow

% Right-shifted relation symbols for alignment with :=
\newcommand\crel[1]{\mathrel{\hphantom:{#1}}}
\newcommand\isom{\crel\cong}
\newcommand\eqls{\crel=}

